ProxEmo: Gait-based Emotion Learning and Multi-view Proxemic Fusion for Socially-Aware Robot Navigation

We present ProxEmo, a novel end-to-end emotion prediction algorithm for socially aware robot navigation among pedestrians. Our approach predicts the perceived emotions of a pedestrian from walking gaits, which is then used for emotion-guided navigation taking into account social and proxemic constraints. To classify emotions, we propose a multi-view skeleton graph convolution-based model that works on a commodity camera mounted onto a moving robot. Our emotion recognition is integrated into a mapless navigation scheme and makes no assumptions about the environment of pedestrian motion. It achieves a mean average emotion prediction precision of 82.47% on the Emotion-Gait benchmark dataset. We outperform current state-of-art algorithms for emotion recognition from 3D gaits. We highlight its benefits in terms of navigation in indoor scenes using a Clearpath Jackal robot.

==> 3-Overview.tex <==
% \section{Overview and Methodology}\label{overview}
% \label{Sec:Overview}

% We propose a novel approach for classifying emotions from gaits that works with an egocentric camera setup. Our method uses 3D poses of human gaits obtained from a camera on the robot to classify perceived emotions. These perceived emotion tags are then used to perform socially aware navigation through a pedestrian environment. \\

% Figure \ref{fig:overview} illustrates our overall pipeline for navigation. Frames extracted from an onboard camera are first processed for pose extraction. The change in pose is then tracked frame by frame for a specified time, and encoded into an image. The resultant embedded image is then fed into our {\algoname} model, which computes the emotion for all the humans in a current scene. Figure~\ref{fig:vs_gcnn} shows our GCN model for emotion classification. The network keeps track of different views of skeletal data through group convolution layers. A softmax on the prediction from each group provides the emotional state. Finally, the perceived emotions obtained are fed into a decentralized collision avoidance algorithm that combines the emotion data via proxemic constraints with LIDAR scans to perform socially aware navigation in a pedestrian environment.
% The data is widely distributed across the four categories with the Happy category containing the largest number of gaits with 32.07\% and the Neutral category containing the smallest number of gaits with 16.35\%. The dataset is collected with subjects from a variety of ethnic backgrounds in both indoor and outdoor environments.

